Understanding Knowledge Drift in LLMs through Misinformation

Large Language Models (LLMs) have revolutionized numerous applications, making them an integral part of our digital ecosystem. However, their reliability becomes critical, especially when these models are exposed to misinformation. We primarily analyze the susceptibility of state-of-the-art LLMs to factual inaccuracies when they encounter false information in a QnA scenario, an issue that can lead to a phenomenon we refer to as *knowledge drift*, which significantly undermines the trustworthiness of these models. We evaluate the factuality and the uncertainty of the models' responses relying on Entropy, Perplexity, and Token Probability metrics. Our experiments reveal that an LLM's uncertainty can increase up to 56.6% when the question is answered incorrectly due to the exposure to false information. At the same time, repeated exposure to the same false information can decrease the models uncertainty again (-52.8% w.r.t. the answers on the untainted prompts), potentially manipulating the underlying model's beliefs and introducing a drift from its original knowledge. These findings provide insights into LLMs' robustness and vulnerability to adversarial inputs, paving the way for developing more reliable LLM applications across various domains. The code is available at https://github.com/afastowski/knowledge_drift.

==> sections/related_works_old.tex <==
\section{Related Work}\label{sec:sota}

%Sycophantic behavior (though not a major focus in this paper, more a side-effect we're trying to circumvent): \cite{wei2024simple}, \cite{sharma2023understanding}, \cite{ranaldi2023large}\newline
%Uncertainty metrics for natural language generation (for sequences): \cite{chen2024inside}


Previous research has extensively explored the capabilities of language models in various NLP tasks. For example,~\cite{brown2020language} introduced GPT-3, demonstrating its ability to perform diverse tasks through few-shot learning. This model's performance in open-domain question-answering tasks has been particularly notable, setting new benchmarks in several datasets, including TriviaQA.

\emph{Uncertainty estimation in language models} that build on deep-learning architectures has also been a subject of significant interest. Gal and Ghahramani~\cite{gal2016dropout} proposed using dropout as a Bayesian approximation to estimate uncertainty in deep learning models. Hendrycks and Gimpel~\cite{hendrycks2017baseline} introduced baseline methods for detecting misclassification through uncertainty estimation. These techniques have been applied to NLP models to estimate their confidence in generated outputs, providing a measure of reliability.

\emph{Adversarial attacks on language models} represent another critical study area. Jia and Liang~\cite{jia2017adversarial} demonstrated that adversarial examples could easily fool NLP models by subtly altering the input to produce incorrect outputs. This has prompted research into developing more robust models capable of withstanding such manipulations. Our work builds on these studies by specifically focusing on how false information affects a model's answer correctness and uncertainty.

\emph{Sycophancy in language models} has been the subject of many recent studies reporting that models often produce agreeable responses that align with input biases, even if factually incorrect. For example, \cite{ranaldi2023large,huang2023survey,park2024ai} have highlighted that LLMs tend to agree with misleading information, reflecting a vulnerability that can be exploited to spread misinformation. These findings underscore the need for models to critically assess and counter false inputs to maintain reliability and factual accuracy.

\emph{The integration of human feedback and fine-tuning in language models} has focused on enhancing their robustness and reliability by incorporating human feedback through reinforcement learning, learning-to-rank, and fine-tuning mechanisms~\cite{stiennon2020learning,ouyang2022training,bai2022training,rafailov2024direct,yang2024crowdsourcing}. The goal of all these approaches is to teach the model to return answers that are in line with the user's intentions and preferences, societal norms, and factual correctness, thus improving the trustworthiness and usability of the language models in real-world applications.

\emph{Model architectures} have improved significantly in recent years. Raffel et al.~\cite{raffel2020exploring} introduced the T5 model, treating all NLP tasks as text-to-text problems, which led to significant improvements across various benchmarks and influenced subsequent model architectures. Liu et al.~\cite{liu2019roberta} presented the RoBERTa model, setting new standards for pre-training and fine-tuning and achieving substantial gains in NLP tasks. Based on these findings and insights, current language models, particularly closed-source ones, have advanced significantly. However, understanding the strategies employed to enhance their reliability remains challenging due to the proprietary nature of these models.
